ICONA: Inter Cluster ONOS Network Application

Several Network Operating Systems (NOS) have been proposed in the last few years for Software Defined Networks; however, a few of them are currently offering the resiliency, scalability and high availability required for production environments. Open Networking Operating System (ONOS) is an open source NOS, designed to be reliable and to scale up to thousands of managed devices. It supports multiple concurrent instances (a cluster of controllers) with distributed data stores. A tight requirement of ONOS is that all instances must be close enough to have negligible communication delays, which means they are typically installed within a single datacenter or a LAN network. However in certain wide area network scenarios, this constraint may limit the speed of responsiveness of the controller toward network events like failures or congested links, an important requirement from the point of view of a Service Provider. This paper presents ICONA, a tool developed on top of ONOS and designed in order to extend ONOS capability in network scenarios where there are stringent requirements in term of control plane responsiveness. In particular the paper describes the architecture behind ICONA and provides some initial evaluation obtained on a preliminary version of the tool.

==> acronyms.tex <==
% For articles we don't need the environment,
% just the list with acrodef's

\acrodef{ide}[IDE]{Integrated Development Environment}
\acrodef{odl}[ODL]{OpenDayLight}
\acrodef{sdn}[SDN]{Software-Defined Networking}
\acrodef{sw}[SW]{Software}
\acrodef{netide}[NetIDE]{NetIDE}\acused{netide}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-PDF-mode: t
%%% TeX-master: "netide"
%%% End:


==> macros.tex <==
\newcommand{\reffig}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsec}[1]{Section~\ref{section:#1}}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-PDF-mode: t
%%% TeX-master: "netide"
%%% End:


==> results-old.tex <==
\section{Evaluation}\label{section:results}

The purpose of the experimental tests described in this section is to compare ICONA with a standard ONOS setup, and evaluate the performances of the two solutions in an emulated environment.

The control plane is always composed of 8 virtual machines, each with four Intel Core i7-2600 CPUs @ 3.40GHz and 8GB of RAM. While for the ONOS tests all the instances belong to the same cluster, with ICONA we have created 2, 4 and 8 clusters, respectively with 4, 2 and 1 instances each. 
The data plane is emulated by Mininet \cite{mininet} and Netem \cite{netem}: the former creates and manages the OpenFlow 1.3 network, while the latter emulates the properties of wide area networks, such as variable delay, throughput and packet loss. Both solutions (ONOS and ICONA) have been tested with both a regular (grid) topology and with the topology of the G\'EANT \cite{geant} pan-European network. 
It is important to highlight that the current ONOS release (Avocet 1.0.1) is focusing on functions and correctness, while Blackbird, to be released in March, will dramatically improve the internal performance. For these reasons, the results presented in this section should not be considered as benchmark.

\begin{figure}
\centering
\includegraphics[width=.30\textwidth]{grid.pdf}
\caption{4*4 grid network with single ONOS cluster (red) and ICONA with 4 clusters (green - two of four displayed), and the one-way delays between data and control planes. Each ICONA cluster is displayed with green dotted lines.}
\label{fig:grid}
\end{figure}

\subsection{Reaction to Network Events}
\subsubsection{Grid networks}

The first performance metric is end-to-end latency of the system for updating the network state in response to events; examples include rerouting traffic in response to link failure or moving traffic in response to congestion.
To evaluate how the system performs when the forwarding plane scales-out, we have selected some standard grid topologies, with a fixed link delay of 5ms (one-way). By network design (the control and data network share the same topology), the average delay between the data and the control planes increases while the physical network is growing. Indeed, it's a function of the number of devices and the delays between them and the ONOS cluster that is located in a central position. However, having multiple clusters interconnected with ICONA decreases the average delay between each cluster and the controlled network. Figure \ref{fig:grid} shows a 4*4 grid topology, with ONOS (red) and ICONA configured with 4 clusters (green, only two of four clusters shown), and the delays between the data and control planes. With ICONA, the delay is always 5ms, while for ONOS it changes from 5 to 15 ms, due to the greater distance between the switches and the cluster. Similar results can be obtained having two or eight ICONA clusters managing the same data plane. The work in \cite{placement} proposes some formulas that explain how the control plane latency is strictly dependent from the network size and delay.


 \begin{figure}
\centering
\includegraphics[width=.48\textwidth]{plot.pdf}
\caption{Average, maximum and mininum latency to reroute 100 paths in case of link failure for ONOS and ICONA (2, 4 and 8 clusters)}
\label{fig:res_grid}
\end{figure}

It is worthwhile to highlight that the number of VMs composing the control plane is always the same (e.g. eight), independently of the data plane dimension and the number of clusters.
One thousand paths are installed in the network. At a certain point, a link, in which one hundred pseudo-wires are running, fails. 
We define as overall latency the amount of time that both ONOS and ICONA require to react to the failure as the sum of: i) the amount of time for the OpenFlow messages (\texttt{PORT\_STATUS} and \texttt{FLOW\_MOD}) to traverse the control network, ii) the alternative path computation, iii) the installation of new flows in the network devices and iv) the deletion of the pre-existing flows. 
Figure \ref{fig:res_grid} shows the latency (avg, min, max) required for the different solutions to execute the four tasks previously mentioned. Each test has been repeated 20 times. Despite the same mechanism used by ICONA to compute and install the new paths, we believe the difference is due to two main reasons: i) each ICONA cluster is closer to the devices, thus reducing the amount of time required for OpenFlow messages to cross the control channel and ii) the ICONA clusters are smaller, with fewer links and devices, thus decreasing the computation time and the overall numbers of flows to be installed and removed from the data plane.



\subsubsection{GEANT network}

The same metrics have been evaluated on the G\'EANT topology (see Figure \ref{fig:geant}). 
Circuits have various one-way delays (from 10 to 50ms) and throughputs (from 1 to 100Gbps). 
 
 \begin{figure}
\centering
\includegraphics[width=.40\textwidth]{geant.pdf}
\caption{G\'EANT pan-European network }
\label{fig:geant}
\end{figure}

\begin{table}[h]
%\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{|p{1.5cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|}
\hline
\textbf{Control plane} & \textbf{Avg latency [ms]} & \textbf{Min latency [ms]} & \textbf{Max latency [ms]} \\ \hline
ONOS     &          297           & 284   & 308  \\ \hline
ICONA2         & 272          & 261 &   296  \\ \hline
ICONA4         & 246          & 232 &   257  \\ \hline
ICONA8           & 221          & 199 &   243  \\ \hline
\end{tabular}
\end{center}
\caption{G\'EANT network: average, maximum and mininum latency to reroute 100 paths in case of link failure for ONOS and ICONA (2, 4 and 8 clusters)}
\label{tab:geant_res}
\end{table}

Table \ref{tab:geant_res} depicts similar results as the previous test. 
ONOS has been compared with three different ICONA deployments, with 2, 4 and 8 clusters, respectively with 4, 2 and 1 instances each. While having the same number of VMs running the control plane software, their geographical distribution improves the overall performance of the system.
While the network is smaller than the 10*10 grid topology, with 41 switches and 58 bi-directional links, the higher delay in the data plane requires an additional amount of time to reconverge.


\subsection{Startup Convergence Interval}
This second experiment measures the overall amount of time required for both solutions to re-converge after a complete disconnection between the control and data planes. The tests have been performed over the G\'EANT topology, and replicated 20 times. Table \ref{tab:start_res} shows the average, maximum and minimum values in seconds. 

\begin{table}[h]
%\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{|p{1.5cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|}
\hline
\textbf{Control plane} & \textbf{Average Time [s]} & \textbf{Minimum Time [s]} & \textbf{Maximum Time [s]} \\ \hline
ONOS    &          6,98           & 6,95  & 7,06   \\ \hline
ICONA           &      6,96       &  6,88 & 7,02    \\ \hline
\end{tabular}
\end{center}
\caption{Amount of time required to obtain the network convergence after disconnection for ONOS and ICONA}
\label{tab:start_res}
\end{table}

The result shows that ICONA and ONOS require comparable time intervals to return to a stable state, in case of a complete shutdown or a failure of the control plane.

